A Unified Comparison of User Modeling Techniques for Predicting Data Interaction and Detecting Exploration Bias

The visual analytics community has proposed several user modeling algorithms to capture and analyze users' interaction behavior in order to assist users in data exploration and insight generation. For example, some can detect exploration biases while others can predict data points that the user will interact with before that interaction occurs. Researchers believe this collection of algorithms can help create more intelligent visual analytics tools. However, the community lacks a rigorous evaluation and comparison of these existing techniques. As a result, there is limited guidance on which method to use and when. Our paper seeks to fill in this missing gap by comparing and ranking eight user modeling algorithms based on their performance on a diverse set of four user study datasets. We analyze exploration bias detection, data interaction prediction, and algorithmic complexity, among other measures. Based on our findings, we highlight open challenges and new directions for analyzing user interactions and visualization provenance.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/methods.tex <==
\section{Methods and Materials}
\label{sec:methods}



We compare a total of eight user models, based on a variety of theoretical approaches and summarized in \autoref{tab:methods-overview}. This section describes our notation, the algorithms, datasets, and the performance measures.  

\subsection{User Modeling Methods}
To form our collection of algorithms discussed in this paper, we started with the pool of papers that were discussed in Xu et al.'s~\cite{xu2020survey} 2020 survey on the analysis of user interactions and provenance in visual analytics. We accounted for the papers published around the same time and after the survey by performing a forward citation search on the manuscripts in the survey and the survey itself. We narrowed the pool to the final selection of seven papers\cite{ottley2019follow, wall2017warning, monadjemi2020competing, gotz2016adaptive, monadjemi2020active, healey2012interest, zhou2021modeling} based on the criteria described in \autoref{sec:scope}, each including algorithms for either learning information relevance or bias detection from observing data interactions. Of the algorithms we selected, three can only infer information relevance (\textit{k}-Nearest Neighbors\cite{monadjemi2020active}, Boosted Naive Bayes\cite{healey2012interest}, and Analytic Focus \cite{gotz2016adaptive} ), two can only detect bias (Attribute Distribution Bias Metric\cite{wall2017warning} and Adaptive Contextualization\cite{gotz2016adaptive}), and two can infer both (Hidden Markov Model\cite{ottley2019follow} and Competing Models\cite{monadjemi2020competing}). In addition to the selected algorithms, we also introduce and provide the performance of an ensemble model which was developed with all the modeling techniques mentioned above that infer information relevance. We provide their algorithmic details below.

% \begin{table}[!b]
%     \centering
%     \caption{Notations and sets used in this paper.}
%     \begin{tabular}{p{0.43\linewidth} p{0.48\linewidth}}
%         \toprule
%          Set Notation & Description \\
%          \midrule
%          ${\mathcal{D} = \{x_1, x_2, ..., x_n\}}$ & The set of underlying data points visualized. \\
%          \midrule
%          ${\mathcal{A} = \{a_1, a_2, ..., a_d\}}$ & The set of attributes (or dimensions) for the underlying data set. \\
%          \midrule
%          $\Alpha = \{\alpha_1, \alpha_2, ...\}$   & The set of possible interactions (e.g.\ hover, click, etc.) \\
%          \midrule
%          ${\mathcal{I} = \{(x_{i, t}, \alpha) \mid t = 1, 2, 3, ...\}}$ & The sequence of interactions in a session. $(x_{i, t}, \alpha)$ denotes taking action $\alpha$ on data point $x_i$ at time step $t$. \\
%          \bottomrule
%     \end{tabular}
%     \label{tab:set_descriptions}
% \end{table}

\subsubsection{Inferring Information Relevance}
This category of algorithms aims to learn users' latent data interest and rank data points based on this interest. Given this ranking, a common applications are attention tracking and next click prediction\cite{monadjemi2020active,monadjemi2020competing,ottley2019follow}. We define the \emph{relevance function} as follows:
\begin{equation}
    \label{eq:f_rank}
    f_{r} \colon \mathcal{D} \mapsto [0, 1],
\end{equation}
where the set of data points, $\mathcal{D}$, is mapped to a numerical value between 0 and 1. Higher values correspond data points being more relevant to the task at hand.
Given two data points $x_i, x_j \in \mathcal{D}$, we say $x_i$ is more relevant to the task at hand, $x_i \succ x_j$, if it has a higher relevance value, $f_{r}(x_i) \textgreater f_{r}(x_j)$.


%%
%% kNN
%%
\vspace{1em}
\noindent
\textbf{\textit{k}-Nearest Neighbors Classifier} as seen in \cite{monadjemi2020active}:
\vspace{0.5em}

\noindent
%overview
A straightforward method for learning users' data interest by observing interactions is to train a $k$-nearest neighbors (\knn) binary classifier. 
%assumptions
\textbf{This approach assumes that proximity drives a user's exploration patterns.}
Monadjemi et al.\cite{monadjemi2020active} built a \knn classifier that relies on a notion of distance between data points and computing the matrix of $k$ nearest neighbors for every data point given the defined distance formula as a pre-processing step. The complexity for this pre-processing step is $O(n^{2}d)$. Refer to \autoref{tab:methods-overview} for more information and complexity variables. This model assumes that every data point in in the dataset, $x_i \in \mathcal{D}$, has a binary label $y_i \in \{0, 1\}$. 
%details
A label of $y_i=1$ means the data point $x_i$ is relevant to the task at hand, whereas a label of $y_i=0$ means $x_i$ is irrelevant. By considering the labels of the nearest neighbors, this model is able to provide us with the probability of any given point being relevant in light of past observations: $\Pr(y_i=1 \mid x_i, \mathcal{I})$. Hence, we use this posterior belief as our relevance function:
\begin{equation}
    f_r(x_i) = \Pr(y_i=1 \mid x_i, \mathcal{I}).
\end{equation}


%%
%% Naïve Bayes
%%
\vspace{1em}
\noindent
\textbf{Boosted Naive Bayes Classifier} as seen in \cite{healey2012interest}:
\vspace{0.5em}

\noindent
Healey et al.\cite{healey2012interest} propose a naive Bayes classifier for maintaining a belief over users' interest in data points.
%assumptions
This approach tracks the frequencies of attributes explored and \textbf{assumes that the user's latent data interest is related to the dataset attributes' occurrence rate.}
%details
In a similar formulation as the \knn\ approach, each data point $x_i \in \mathcal{D}$ has a binary label $y_i \in \{0, 1\}$. A label of $y_i = 1$ means the point $x_i$ is relevant to the task at hand and a label of $y_i = 0$ means it is not relevant. The goal of this approach is to reason about the unknown labels in light of frequencies of observations calculated via the Bayes' law:
\begin{equation}
    \Pr(y_i=1 \mid x_i) \propto \Pr(x_i \mid y_i = 1)\Pr(y_i=1).
\end{equation}
Extending $x_i$ to each of its individual $d$ dimensions and assuming conditional independence among attributes, we get:
\begin{equation}
\begin{split}
        &\Pr(y_i=1 \mid x_{i, 1}, x_{i, 2}, ..., x_{i, d})\\ 
        \propto &\Pr( x_{i, 1}, x_{i, 2}, ..., x_{i, d} \mid y_i = 1)\Pr(y_i=1) \\
        = & \Pr(y_i=1) \prod_{j=1}^{d} \Pr(x_{i,j} \mid y_i=1),
\end{split}
\end{equation}
where $x_{i, j}$ denotes the $j$th attribute of the $i$th data point. Therefore, we get the relevance function as:
\begin{equation}
    f_r(x_i) = \Pr(y_i=1) \prod_{j=1}^{d} \Pr(x_{i,j} \mid y_i=1).
\end{equation}

%This model is called \emph{naive} because of the conditional independence assumption among attributes. %In more sophisticated models, the dependencies among variable are leaned via techniques called Bayesian structure learning. 
While Naive Bayes often performs as well as more sophisticated models in practice \cite{langley1992analysis}, its performance can further be improved by \emph{boosting}. As recommended by Healey et al.\cite{healey2012interest}, we used AdaBoost to train a stronger classifier.





%%
%% Analytic Focus Modeling
%%
\vspace{1em}
\noindent
\textbf{Analytic Focus Modeling} as seen in \cite{zhou2021modeling}:
\vspace{0.5em}

\noindent
Zhou et al.\cite{zhou2021modeling} propose a technique for modeling analytic focus (\af) during a session. Their technique is based on an abstract notion of \emph{concepts} defined as \emph{``meaningful data attribute[s] in the problem domain."} This technique tracks user focus on each of the concepts by observing their interactions and maintain an importance score for each concept.  \textbf{The model assumes that the user's latent interest is related to the occurrence rate of discrete \textit{concepts} observed in their data interactions.}
With concepts being left open for practitioners to define in their particular domain, here, we let each unique value appearing in the discrete attributes of the dataset to represent a concept, performing a pre-processing step on continuous attributes to convert them into discrete bins. 

%\acro{AF} supports different types of interactions. 
Each interaction $\alpha \in \Alpha$ is defined by two values: an initial importance score $I_\alpha(0)$ and a persistence score $P_\alpha$. In a sense, $I_\alpha(0)$ refers to how intentional an action is and how informative it is in revealing analytic focus while $P_\alpha$ is a measure of how long the visual changes resulting from action $\alpha$ remain.
Using these parameters and the Ebbinghaus forgetting curve \cite{ebbinghaus1880urmanuskript,ebbinghaus1885gedachtnis,murre2015replication}, the authors define the per-action importance score function $t$ time steps after an action is taken as: 
\begin{equation}
    I_{\alpha}(t) = I_{\alpha}(0) \times e^{-\frac{t}{P_{\alpha}}}.
\end{equation}
%

Using the equation above, the authors propose an additive model for calculating the importance score for each concept $c$ at time $\tau$:
%
\begin{equation}
    I^c(\tau) = \sum_{(x_{i, t}, \alpha) \in \mathcal{I}_{\tau,c}}I_{\alpha} (\tau - t),
\end{equation}
%
where $\mathcal{I}_{\tau, c}$ denotes the set of interactions with points involving concept $c$ up until time step $\tau$. Considering that each data point $x_i \in \mathcal{D}$ may subscribe to multiple concepts (one concept per dimension in our case), we extend this method so that the importance of a data point is the product of the importance of its individual concepts. In other words, given a data point $x_i \in \mathcal{D}$ and the current time step $\tau$, 
%
\begin{equation}
    f_r(x_i) = \prod_{c \in C(x_i)}{I^c(\tau)},
\end{equation}
%
where $C(x_i)$ is the list of concepts with which $x_i$ is associated.


\subsubsection{Detecting Exploration Bias}
The goal of bias detection is to determine if user interactions are biased towards a certain attribute in the dataset. Detected biases can be used to bring awareness and mitigate users from focusing on a subset of the data~\cite{gotz2016adaptive,wall2017warning,wall2022left}. Additionally, bias detection can be leveraged to infer the user's interest and incorporated into intelligent systems to better aid the user during data exploration. Using a standard notation for every approach considered in this work, we define the \emph{bias function}, $f_{b}$, as follows:
\begin{equation}
    \label{eq:f_bias}
    f_{b} \colon \mathcal{A} \mapsto [0, 1],
\end{equation}
where the set of attributes, $\mathcal{A}$, is mapped to a numerical value between 0 and 1. Higher values correspond to more severe bias towards a certain attribute.


%%
%% Analytic Focus Modeling
%%
\vspace{1em}
\noindent
\textbf{Attribute Distribution Bias Metric} as seen in \cite{wall2017warning}:
\vspace{0.5em}

\noindent
Wall et al.\cite{wall2017warning} propose a set of metrics for quantitatively detecting various types of cognitive biases. The most relevant to our work is the metric they call \emph{attribute distribution} bias. 
\textbf{Their approach assumes that in an unbiased exploratory session, the distribution of values explored by the user will resemble the distribution of the underlying data.} It relies on well-known statistical tests, Chi-Square\cite{mchugh2013chi} and Kolmogorov–Smirnov\cite{massey1951kolmogorov}, which are used for discrete and continuous attributes respectively. In each case, the test takes the underlying data as well as the set of points with which the user has interacted as inputs and returns a $p$-value indicating whether or not the two samples could be reasonably drawn from the same distribution. Then, they define their attribute distribution metric for a given attribute $a_i \in \mathcal{A}$ to be:
\begin{equation}
    f_{b}(a_i) = 1 - p\text{-value}_{a_{i}}.
\end{equation}

%%
%% Adaptive Contextualization
%%
\vspace{1em}
\noindent
\textbf{Adaptive Contextualization} as seen in \cite{gotz2016adaptive}:
\vspace{0.5em}

\noindent
Gotz et al.\cite{gotz2016adaptive} propose a metric to measure selection bias in real-time. This methods assumes that you can detect exploration bias by comparing the distributing  


In order to detect such biases, they propose measuring the Hellinger distance between the datasets before and after filtering. Hellinger distance is a statistical measure designed to quantify the similarity between two distributions. Thus, \textbf{this approach assumes that we can detect bias by comparing the observed distribution to the expected data distribution}. The authors propose using the Hellinger distance defined for discrete probability distributions with a pre-processing step to discretize the continuous attribute into discrete bins. 

Consider a particular dimension of interest, $a_i$, represented as a set of $m$ discrete values $\{v_1, v_2, ..., v_m\}$. The distribution of these values in the underlying data and interaction data are $\{p_1, p_2, ..., p_m\}$ and $\{q_1, q_2, ..., q_m\}$ respectively.  We compute the Hellinger distance as:
\begin{equation}
    f_b(a_i) = H(\mathcal{D}_{a_i}, \mathcal{I}_{a_i}) = \sqrt{\frac{1}{2} \sum_{j=1}^{m}{(\sqrt{p_j} + \sqrt{q_j})^2} },
\end{equation}
where $\mathcal{D}_{a_i}$ and $\mathcal{I}_{a_i}$ denote only the $a_i$ attribute of the underlying and interaction datasets respectively. While this technique was intended to detect selection bias (i.e.\ before vs.\ after filtering), we adopt it to quantify exploration bias.

%\ao{move to discussion?}
%This method has the benefit of being non-parametric (hence flexible) and computationally fast to update in light of observations.



\subsubsection{Inferring Both Information Relevance and Exploration Bias}
\label{sec:hmm-cm}


%%
%% Hidden Markov Model
%%
\vspace{1em}
\noindent
\textbf{Hidden Markov Model} as seen in \cite{ottley2019follow}:
\vspace{0.5em}

\noindent
Ottley et al.\cite{ottley2019follow} propose a Hidden Markov Model (\hmm) approach for modeling user attention during visual exploratory analysis. \textbf{Their approach assumes that the visual features of the interface will drive the user's attention (it considers all possible combinations)} and their interactions such that attention at time $t+1$ will be similar to the observation at time $t$ . They constructed a hidden Markov model, presuming the user's behavior evolves under a Markov process (that is, the behavior at a particular time only depends on their behavior at the previous time step), and interaction events are generated conditionally independently given this sequence of attention shifts. The set of visible visual features (\eg\ color, position, size, etc.) creates the \textit{mark space} and the latent states. Further, their algorithm uses particle filtering~\cite{gordon1993novel,doucet2000sequential} to sample from the model's posterior distribution and predict the user's attention for the next time step. Integral to this technique is a \textit{bias vector} that captures the relative importance of the mark space components. We use the particle filter output to predict information relevance and the bias vector for bias detection. 


%\paragraph{Expected Strengths and Limitations?}
%\shayan{Key ideas missing here ares (1) the model is based on visual attributes, (2) the $\pi$ vector for biases, (3) our extension to go beyond visual channels and use every attribute in the data.}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/datasets.png}
    \caption{A summary of the characteristics of the selected user interaction datasets and the performance of the user modeling techniques with said datasets. We represent success using each technique's performance at top-100 points for information relevance.}
    \label{fig:datasets}
\end{figure*}


%%
%% Competing Models
%%
\vspace{1em}
\noindent
\textbf{Competing Models} as seen in \cite{monadjemi2020competing}:
\vspace{0.5em}

\noindent
Monadjemi et al.\cite{monadjemi2020competing} propose a Bayesian model selection approach for detecting exploration bias and inferring information relevance during visual exploratory analysis. This approach, called \emph{Competing Models} (\cm), enumerates a set of probabilistic models each of which represent exploration based on a subset of data attributes. 
Given a dataset with $d$ attributes, they enumerate the model space ${\mathbf{M} = \{\mathcal{M}_1, \mathcal{M}_2, ..., \mathcal{M}_{2^d}\}}$ where each model represents exploration based on one subset of attributes. \textbf{Thus, it assumes and one or more data attributes (it considers all possible combinations) are sufficient to represent a users data interest.} As interactions arrive, they maintain a belief ${\Pr(\mathcal{M}_i \mid \mathcal{I})}$ which is interpreted as the viability of model $\mathcal{M}_i$ in explaining user interactions.
To infer the relevance of data points to the task at hand in light of past interactions, they use Bayesian model averaging to get:
\begin{equation}
    f_r(x_i) = \Pr(x_i \mid \mathcal{I}) = \sum_{j=0}^{2^d}\Pr(x_i \mid \mathcal{I}, \mathcal{M}_j).
\end{equation}
%
To quantify bias towards each attribute, they use the law of total probability as follows:
\begin{equation}
    f_b(a_i) = \sum_{\mathcal{M}_j \in \mathbf{M}_{a_i}} \Pr(\mathcal{M}_j \mid \mathcal{I}),
\end{equation}
where $\mathbf{M}_{a_i} \subset \mathbf{M}$ denotes the set of models involving attribute $a_i$.


\subsubsection{Inferring Information Relevance via an Ensemble Approach}

%%
%% Ensemble
%%
\vspace{1em}
\noindent
\textbf{Ensemble Model}
\vspace{0.5em}

\noindent
We anticipate that no model will be able to correctly recognize relevant points in every system, task, or dataset. This phenomena was also observed by the machine learning community which led to the development of \emph{ensemble methods} \cite{rokach2010ensemble,dietterich2000ensemble}. Ensembles are a collection of classification models combined to construct a model with higher predictive power. Using this approach, we consider a final technique which combines predictions from all five techniques that infer information relevance reviewed in this paper. For a given data point, $x_i \in \mathcal{D}$, we compute the relevance function, $f_r(x_i)$, using each of the modeling techniques and average the relevance values to get the ensemble prediction. Then, we proceed with ranking the data points according to their relevance, a process identical to the one in the preceding modeling techniques. 

\subsection{User Study Datasets}
\label{sec:datasets}
We used four publicly available datasets from user study experiments with visualization systems. These studies contained varying interfaces as well as task designs. We aimed to evaluate and compare the performance of the user modeling techniques with a variety of interaction logs, ranging from studies with very directed and specific tasks to the polar opposite, open data exploration. Refer to  ~\autoref{fig:datasets} for a detailed summary of the characteristics of each dataset.

\subsubsection{Directed User Studies}
Although the user studies in this section are directed, they differ in the intensity of direction a user was provided while performing the task. We describe the user studies in more detail below.

\vspace{1em}
\noindent
\textbf{STL Crimes} as seen in \cite{ottley2019follow}:
\vspace{0.5em}

\noindent
The \textit{STL Crimes} dataset \textbf{involved a highly specified task thus capturing less exploration noise. We selected this dataset as it represents the best-case observational scenario for user modeling.}



Curated by Ottley et al.~\cite{ottley2019follow}, %the St. Louis Crime dataset was pulled from the database of crimes maintained by the Metropolitan Police Department of St. Louis \cite{Crime}. 
this dataset consists of 1,951 crime instances reported in the month of March 2017 with a total of eighteen attributes. Each instance of crime on the map was displayed as a dot with a position and color, indicating the location and type of the crime respectively. Eight types of crime exist in the database: homicide, theft-related, assault, arson, fraud, vandalism, weapons, and vagrancy.  30 participants were recruited from Mechanical Turk and they completed three categories of directed search tasks that were designed to encourage them to either click on: (1) \textit{Type-Based} data points with similar crime categories (e.g. Homicide, Assault, etc.), (2) \textit{Location-Based} data points that are within in the same vicinity, or (3) \textit{Mixed} data points that are of the same crime category and in the same vicinity. Each participant completed a total of six tasks, two from each category. Since the authors specified to the participants target attributes to interact with, this provides us with a notion of ground-truth bias. In their user study, Ottley et al.~\cite{ottley2019follow} captured mouse click data as participants interacted the visualization. Consistent with Ottley et al.~\cite{ottley2019follow}, we filtered the data to hold only the interactions of participants who successfully answered the task questions and created three data subsets: 28 user sessions for location-based tasks, 23 for typed-based, and 27 for mixed. 


\vspace{1em}
\noindent
\textbf{Vastopolis} as seen in \cite{monadjemi2020active}:
\vspace{0.5em}

\noindent
We selected the \textit{Vastopolis} dataset because of the attributes in the dataset. \textbf{It is the only user interaction dataset in this study that includes unstructured text.}

Inspired by the 2011 VAST Challenge, Monadjemi et al.'s~\cite{monadjemi2020active} study describes a major epidemic that started in the fictitious city of Vastopolis. Participant's interacted with a map of Vastopolis with 3000 geolocated tweet-like data. In addition to the social media posts, the map display major roadways, waterways, and landmarks in the city. They recruited 130 participants from Amazon Mechanical Turk and tasked each participant to search through the dataset of microblogs via an interactive map and bookmark as many posts containing illness-related information as possible. Following the same pre-processing step as the authors, 74 user interaction logs remained from the control group of the study. The only interaction type we considered in the interaction logs were intentional ``bookmarks" of the microblogs.


\vspace{1em}
\noindent
\textbf{Political Committee} as seen in \cite{wall2022left}:
\vspace{0.5em}

The \textit{Political Committee} user study \textbf{examined cognitive and exploration bias as participants selected their picks for a hypothetical committee. Thus we selected this dataset as a candidate for examining exploration bias.}


\noindent
Wall et al.~\cite{wall2022left} generated a dataset of 180 fictitious politicians, representing the composition of the Georgia General Assembly. The dataset contains three discrete and six continuous attributes that characterizes each politician. In the study conducted by Wall et al.~\cite{wall2022left}, the authors had users interact with an visualization system that supports the exploration of the fictitious political committee data. There were two versions of the visualization system: a Control version of the interface, and an Intervention version of the interface, which was modified to visualize traces of the user’s interactions with the data in real-time. To assess the effectiveness of visualizing the user's interaction traces, the authors performed an in-lab study with 24 participants. They were tasked with selecting a committee of 10 candidates to review public opinion in Georgia on the controversial bill that bans abortion after 6 weeks. In order to observe the raw, inherent biases of the users, we selected the interaction logs of those in the Control group (total of 12 participants). The authors recorded several types of interactions the user can make with the interface, however, we filtered the interaction log for each user to contain only the interactions when the user ``bookmarked'' a politician to be a part of their political committee. 

\subsubsection{Open-Ended User Study}

%The S\&P 500 Boardrooms dataset comes from the Wall Street Journal~\cite{wsjboardrooms} and it holds various information about the companies and their board of directors in the S\&P 500. The data contains one discrete and six continuous attributes. 

\vspace{1em}
\noindent
\textbf{Boardrooms} as seen in \cite{feng2018effects}:
\vspace{0.5em}

\noindent
The \textit{Boardrooms} study did not involve a particular tasks and instructed the participants to freely interact with the visualisation. \textbf{We expect this dataset to include the highest levels of exploration noise. }

Feng et al.~\cite{feng2018effects,feng2018patterns} utilized the visualization, ``Inside America’s Boardroom," which was published by the \textit{Wall Street Journal}~\cite{wsjboardrooms} in 2016. This point-based visualization displays seven different attributes to the user: market capitalization, ratio of unrelated board members, ratio of female board members, average age of board members, average tenure of board members, and median pay of board members. The study adopted an open-ended approach and observed the user's interactions as they explored the dataset through the visualization.  The interaction log contains a succession of hovers each user made on different data points. To account for unintentional hovers, we followed the same approach as Monadjemi et al.~\cite{monadjemi2020competing}, each user's session was filtered only include hovers that lasted for over one second. Additionally, we only considered sessions that consisted of more than three hovers, resulting in a total of 39 user sessions. 

\subsection{Evaluation Measures}
In this section, we describe the performances measures we used to evaluate the modeling technique on information relevance and bias detection. 

\subsubsection{Information Relevance}

We developed a standardized probabilistic output for each algorithm to directly compare the models to each other. Specifically, techniques treat every data point as a potential candidate for being most relevant to the user data interest. Thus, each method outputs the relevance probability for each data point given a set of interaction observations. This output represent the technique's unique interpretation of information relevance. For example, \knn\ assumes that the data points most relevant to the user will minimize some measure of distance while \af\ examines the frequency on \textit{concepts} from the past interactions. 


In our evaluation, ground truth relevance is unobservable. Still, we used the next interaction as a proxy, presuming that the user will interact with the data points they perceive to be most relevant to their task. 
Given the model's probabilities, we can rank each data point based on algorithm's information relevance belief.
We report \topk\ data retrieval for the algorithms for $\kappa \in \{1,5,10,20,50,100\}$ which we will refer to as the \textit{prediction sets}. We considered a variety of set sizes. For example, an alternative is to use percentages instead of a fixed values. However, for large datasets, retrieving a small percentage to the dataset can still be overwhelming to the user if we consider the goal of provided real-time analysis support. This standardized output enables us to evaluate and compare each technique's ability to infer information relevance.

We record the following measures for every observed interaction the datasets:
\vspace{-.5em}
\begin{itemize}[noitemsep]
    \item \textbf{\success:} $\in \{0,1\}$, binary value for whether the next interaction was included in the prediction set for all values of $\kappa$.
    \item \textbf{\rank:} the ranked position of the next observed interaction such that lower is better.
\end{itemize}



%Emulating on the evaluation method from Ottley et al. and Monadjemi et al.~\cite{ottley2019follow, monadjemi2020competing}, we use $\kappa = \{1,5,10,20,50,100\}$.
% The second metric measures the rank at which the predicted interaction was positioned in the prediction set for each model (lower is better).


%, we captures represents the mean rank of the true interaction in the ranking of possible interactions according to the model (lower is better).

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/Lima.png}
    \caption{Comparing participant Lima's interactions (foreground) to the full dataset distribution (background). Both coders reported no significant difference between the two distributions, thus indicating that no bias detected. We observed similar result for all twelve study participants from \cite{wall2022left}.}
    \label{fig:exampleuser}
\end{figure}

\begin{figure*}[!ht]
     \centering
     \begin{subfigure}[b]{.95\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ncp_results.png}
         %\caption{Average \textbf{success rate} across all the tasks in each user study dataset for varying values of the prediction set size.}
         \vspace*{3mm}
     \end{subfigure}
     %
     \begin{subfigure}[b]{.95\textwidth}
        \vspace{-1em}
         \centering
         \includegraphics[width=\textwidth]{figures/ranking_results.png}
         %\caption{Average \textbf{rank} of the next interaction point of the user modeling techniques.}
     \end{subfigure}
     \caption{We evaluated each model's performance with two metrics: (top) Average \textbf{success rate} across all the tasks in each user study dataset for varying values of the prediction set size and (bottom) Average \textbf{rank} of the next interaction point of the user modeling techniques.}
     \label{fig:inference}
\end{figure*}

\subsubsection{Exploration Bias Detection}
\label{sec:bias_detection_gt}

Evaluating each technique's ability to detect exploration bias poses a unique challenge, in that \textit{ground truth} is not always readily available. When evaluating information relevance, we had access to a notion of \emph{success}: we wanted to predict next data points with which the user interacts, and we were able to verify our ability to do so by observing the next interaction point. For bias selection, however, such ground truth is not as easy to access, especially for user study datasets with open-ended tasks. With the \textit{Political Committee} dataset collected by Wall et al.~\cite{wall2022left}, for example, each user can exhibit their own set of biases as they explore the data. 

For this set of evaluations, we use two datasets: \textit{STL Crimes} separated into \textit{location-based}, \textit{type-based}, and \textit{mixed} subsets and \textit{Political Committee}. The \textit{STL Crimes} user study involved a directed task, asking participant to interaction with specific portions of the data. We used the specific task as the ground truth. In our evaluation, an algorithm successfully detects exploration bias if its outputs indicate data attributes related to crime location, type, or a mixture model of type and location for \textit{location-based}, \textit{type-based}, and \textit{mixed} respectively. 

For the \textit{Political Committee}, two researchers performed qualitative coding on each study participants' committee selections, following best practices~\cite{brod2009qualitative}. We used an iterative approach. First, the coders reviewed a single participant's selections and density plots showing the attribute distributions for a given set of interaction logs and the original data distribution. Their goal was to identify evidence of data bias in the observed selections. Next, they established a codebook from this first round and independently coded all twelve participants' interaction logs. After inspecting each of the twelve study participants, both coders agreed the was no observable bias in the interaction study. For example, \autoref{fig:exampleuser} compares study participant Lima's data selection to the individual attribute distribution. Although the coding sessions detected no bias, we included this analysis to assess the algorithms' performance in detecting bias when none exists. 


% Inspired by \ad~\cite{wall2017warning}, we set some notion of ground-truth by stating that the ground-truth bias can be determined by assessing whether the distribution of values explored by the user resembles the underlying data distribution. In order to do so, we used the Chi-Square and Kolmogorov–Smirnov test for discrete and continuous attributes, respectively. If the dataset does not meet the assumptions of the Chi-Square test, we used the Fisher's exact test to retrieve a $p$-value, which indicates whether or not the two samples could be reasonably drawn from the same distribution. If the $p$-value for a given attribute is less than $\alpha = 0.05$, we set the attribute as being one of the top biases of the user at that point in time of interaction. We then evaluate the techniques by comparing the set of ground-truth biases with the top-ranking biases found by each technique.

==> sections/old_versions/selected_datasets.tex <==
\section{Selected User Study Datasets}
\label{sec:datasets}

% \shayan{An overview of what characteristics we looked for when choosing user study datasets. Then details (scenario, visualization, participants, etc.) in each subsection below.}

\ao{I like the structure of this section. Let's do something similar for the algorithms. See \autoref{sec:methods}}
To compare the performance of the selected user modeling techniques, we chose four user study datasets. The selection of datasets we chose vary in the number of visual attributes shown to the user and the degree of openness of the task(s) the user was asked to perform. In this section, we provide an overview of each of the underlying data as well as details of its corresponding user study interaction log. See to Table~\ref{tab:user_study_data} for detailed statistics characterizing the selected user interaction log datasets.

\subsection{St. Louis Crimes}
\subsubsection{Description of the Underlying Data}
The St. Louis Crime dataset was pulled from the database of crimes maintained by the Metropolitan Police Department of St. Louis \cite{Crime}. This dataset consists of 1,951 crime instances committed in the month of March 2017 with a total of eighteen attributes. 

\subsubsection{Description of the Interaction Data}
In their user study, Ottley et al.~\cite{ottley2019follow} captured mouse click data as participants interacted with a crime map visualization of St. Louis. Each instance of crime on the map was displayed as a dot with a position and color, indicating the location (denoted by \textit{longitude} and \textit{latitude}) and \textit{type} of the crime respectively. Eight types of crime exist in the database: homicide, theft-related, assault, arson, fraud, vandalism, weapons, and vagrancy. 30 participants were recruited from Mechanical Turk and they completed three categories of directed search tasks that were designed to encourage them to either click on: (1) \textit{Type-Based} data points with similar crime categories (e.g. Homicide, Assault, etc.), (2) \textit{Location-Based} data points that are within in the same vicinity, or (3) \textit{Mixed} data points that are of the same crime category and in the same vicinity. Their participants completed two tasks for each category, resulting in a total of six tasks. The tasks presented to the participants were:
\begin{enumerate}[noitemsep]
    \item Type-Based: examine data points with similar crime categories
    \begin{enumerate}[noitemsep]
        \item Out of all the cases of Homicide, one case differs from the other cases with regard to time. What is the time of that case?
        \item How many cases of arson occur during PM?
    \end{enumerate}
    \item Location-Based: examine data points that are within in the same vicinity
    \begin{enumerate}[noitemsep]
        \item There are four types Theft-Related crime in the red shaded region: Larceny, Burglary, Robbery and Motor Vehicle Theft. Count the number of cases of Robbery in the red shaded region.
        \item There are two types of Assault: Aggravated and Non-Aggravated assault. Count the number of Non-Aggravated Assault in the red shaded region.
    \end{enumerate}
    \item Mixed: examine data points that are of the same crime category and in the same vicinity
    \begin{enumerate}[noitemsep]
        \item Count the number of crimes that occur during 7:00 AM - 12:30 PM in the red shaded region.
        \item Count the number of crimes during AM in the red shaded region.
    \end{enumerate}
\end{enumerate}
Questions (1) and (2) were type-based tasks, (3) and (4) were location-based tasks and (5) and (6) were mixed tasks. Consistent with Ottley et al.~\cite{ottley2019follow}, we filtered the data to hold only the interactions of participants who successfully answered the task questions, resulting in 28 user sessions for location-based tasks, 23 for typed-based, and 27 for mixed.

\subsection{S\&P 500 Boardrooms}
\subsubsection{Description of the Underlying Data}
The S\&P 500 Boardrooms dataset comes from the Wall Street Journal~\cite{wsjboardrooms} and it holds various information about the companies and their board of directors in the S\&P 500. The data contains one discrete and six continuous attributes. 

\subsubsection{Description of the Interaction Data}
Feng et al.~\cite{feng2018patterns} utilized the visualization, ``Inside America’s Boardroom," which was published by the Wall Street Journal~\cite{wsjboardrooms} in 2016. This point-based visualization displays seven different attributes to the user: \textit{market capitalization, ratio of unrelated board members, ratio of female board members, average age of board members, average tenure of board members, and median pay of board members}. The authors took an open-ended approach to their study and observed the user's interactions as they explored the dataset through the visualization. The interaction log contains a succession of hovers each user made on different data points. To account for unintentional hovers, we followed the same approach as Monadjemi et al.~\cite{monadjemi2020competing}, each user's session was filtered only include hovers that lasted for over one second. Additionally, we only considered sessions that consisted of more than three hovers, resulting in a total of 39 user sessions. 

\subsection{Vastopolis - VAST Challenge 2011}
\subsubsection{Description of the Underlying Data}
In 2011, the Visual Analytics Science and Technology (VAST) community published a fictitious epidemic dataset for their annual challenge. A truck accident over a major river contaminates the water and air with harmful chemicals in the town of Vastopolis. The water flow and wind transport these chemicals to two distinct parts of the city, causing citizens to exhibit symptoms of an illness. This dataset originally contains 1,023,077 microblogs posted on social media from locations around the town during a 21-day period. Monadjemi et al.~\cite{monadjemi2020active} created a subset of this dataset to contain data from the first two days of the epidemic with 33\% of points being related to illness. The authors then picked a random set of 3000 points from this subset to display to users in their study. Each microblog in this dataset is classified to a certain topic keyword based with a labeling heuristic. The data contains one discrete and two continuous attributes. 

\subsubsection{Description of the Interaction Data}
The user study presented in Monadjemi et al.~\cite{monadjemi2020active} involved users in identifying the parts of Vastopolis impacted by the epidemic via analyzing social media posts and their posting location, denoted by \textit{longitude} and \textit{latitude}. The authors recruited 130 participants from Amazon Mechanical Turk and tasked each participant to search through the dataset of microblogs via an interactive map and bookmarking as many posts containing illness-related information as possible. Following the same pre-processing step as the authors, we ended up with a total of 74 user interaction logs from the control group of the study. The only interaction type we considered in the interaction dataset were hovers that lasted at least 500 milliseconds.

\subsection{Political Committee}
\subsubsection{Description of the Underlying Data}
Wall et al.~\cite{wall2022left} generated a dataset of 180 fictitious politicians, representing the composition of the Georgia General Assembly. The dataset contains three discrete and six continuous attributes that characterizes each politician.

\subsubsection{Description of the Interaction Data}
In the study conducted by Wall et al.~\cite{wall2022left}, the authors had users interact with an visualization system that supports the exploration of the fictitious political committee data. There were two versions of the visualization system: a Control version of the interface, and an Intervention version of the interface, which was modified to visualize traces of the user’s interactions with the data in real-time. The goal of interaction traces are to promote reflection and awareness during visual data analysis. To assess the effectiveness of visualizing the user's interaction traces, the authors performed an in-lab study with 24 participants and gave them the following open-ended task: \textit{Imagine you are engaged in political decision-making in the state of Georgia. The debate about abortion is ongoing, with variations of these bills cropping up across other states in the United States, which can potentially learn from the ongoing debate in Georgia. Select a committee of 10 candidates that you feel should review public opinion in Georgia on the controversial Georgia HB481.} For context, the Georgia HB481 bans abortion after 6 weeks (earlier than the previous state law of 20 weeks. In order to observe the raw, inherent biases of the users, we selected the interaction logs of those in the control group (total of 12 participants). The authors recorded several types of interactions the user can make with the interface, however, we filtered the interaction log for each user to contain only the interactions when the user "bookmarked" a politician to be part of their political committee. 

==> sections/old_versions/selected_models.tex <==
With the standardized notation introduced in the preceding section, we now turn our attention to the selection of existing modeling techniques and provide a brief overview for each. Our process for selecting these modeling techniques is simple.We considered every paper cited in a recent survey on analytic provenance in visual analytics by Xu et al\cite{xu2020survey}. In order to account for the papers published after the aforementioned survey, we also considered papers that cited the survey. We narrowed down the pool to the final selection of papers\cite{ottley2019follow, wall2017warning, monadjemi2020competing, gotz2016adaptive, monadjemi2020active, healey2012interest, zhou2021modeling} as each proposed technique either one or both of the two aspects of user modeling we defined in Section\ref{sec:prelims}. Refer to Table~\ref{tab:models} for an overview comparison of the selected modeling techniques.

\subsection{Hidden Markov Model}
Ottley et al.\cite{ottley2019follow} propose a Hidden Markov Model (\acro{HMM}) approach for modeling user attention during visual exploratory analysis. From a high level, their approach is based on the assumption that users interact with nearby points. They construct a probability belief over the set of data points $x_i \in \mathcal{D}$ being involved in the next interaction in light of past observations. Using the Markov property, this probabilistic belief only depends on the last interaction observed. \shayan{Key ideas missing here ares (1) the model is based on visual attributes, (2) the $\pi$ vector for biases, (3) our extension to go beyond visual channels and use every attribute in the data.}

\subsection{Attribute Distribution Bias Metric}
Wall et al.\cite{wall2017warning} propose a set of metrics for quantitatively detecting various types of cognitive biases. The most relevant to our work is the metric they call \emph{attribute distribution} bias. Their approach is based on the assumption that in an unbiased exploratory session, the distribution of values considered by the user resembles the distribution of the underlying data. 

This approach is simple in that it relies on well-known statistical tests. Chi-Square and Kolmogorov–Smirnov tests are used for discrete and continuous attributes respectively. In each case, the test takes the underlying data as well as the set of points with which the user has interacted as inputs and returns a $p$-value indicating whether or not the two samples could be reasonably drawn from the same distribution. Then, they define their attribute distribution metric for a given attribute $a_i \in \mathcal{A}$ to be:
\begin{equation}
    f_{b}(a_i) = 1 - p\text{-value}_{a_{i}}.
\end{equation}

\shayan{Missing ideas: the underlying assumptions for KS and ChiSquare tests, and alternatives when the assumptions are not met.}


\subsection{Competing Models}
Monadjemi et al.\cite{monadjemi2020competing} propose a Bayesian model selection approach for detecting exploration bias and inferring information relevance during visual exploratory analysis. This approach, called \emph{Competing Models}, enumerates a set of probabilistic models each of which represent exploration based on a subset of data attributes. Given a dataset with $d$ attributes, they enumerate the model space ${\mathbf{M} = \{\mathcal{M}_1, \mathcal{M}_2, ..., \mathcal{M}_{2^d}\}}$ where each model represents exploration based on one subset of attributes. As interactions arrive, they maintain a belief ${\Pr(\mathcal{M}_i \mid \mathcal{I})}$ which is interpreted as the viability of model $\mathcal{M}_i$ in explaining user interactions.
%
\shayan{Missing ideas: based on exact inference; not always easy to have; assumptions of the exact inference models. We omit the inner workings of the models in this discussion.} 

To infer the relevance of data points to the task at hand in light of past interactions, they use Bayesian model averaging to get:
\begin{equation}
    f_r(x_i) = \Pr(x_i \mid \mathcal{I}) = \sum_{j=0}^{2^d}\Pr(x_i \mid \mathcal{I}, \mathcal{M}_j).
\end{equation}
%
To quantify bias towards each attribute, they use the law of total probability as follows:
\begin{equation}
    f_b(a_i) = \sum_{\mathcal{M}_j \in \mathbf{M}_{a_i}} \Pr(\mathcal{M}_j \mid \mathcal{I}),
\end{equation}
where $\mathbf{M}_{a_i} \subset \mathbf{M}$ denotes the set of models involving attribute $a_i$.

\subsection{Adaptive Contextualization}
Gotz et al.\cite{gotz2016adaptive} propose a metric to measure selection bias in real-time. Their work was motivated by the fact that, in some scenarios, filtering the dataset by some attributes may introduce unintentional bias towards other attributes. In order to detect such biases, they propose measuring the Hellinger distance between the datasets before and after filtering. Hellinger distance is a statistical measure designed to quantify the similarity between two distributions. The authors propose using the Hellinger distance defined for discrete probability distributions. When working with continuous attributes, they propose a pre-processing step to discretize the continuous domain into discrete bins. Consider a particular dimension of interest, $a_i$, represented as a set of $m$ discrete values $\{v_1, v_2, ..., v_m\}$. The distribution of these values in the underlying data and interaction data are $\{p_1, p_2, ..., p_m\}$ and $\{q_1, q_2, ..., q_m\}$ respectively.  We compute the Hellinger distance as:
\begin{equation}
    f_b(a_i) = H(\mathcal{D}_{a_i}, \mathcal{I}_{a_i}) = \sqrt{\frac{1}{2} \sum_{j=1}^{m}{(\sqrt{p_j} + \sqrt{q_j})^2} },
\end{equation}
where $\mathcal{D}_{a_i}$ and $\mathcal{I}_{a_i}$ denote only the $a_i$ attribute of the underlying and interaction datasets respectively. While this technique was intended to detect selection bias (i.e.\ before vs.\ after filtering), we adopt it to quantify exploration bias.

\subsection{Nearest Neighbors Classifier}
One simple method for learning users' data interest by observing interactions is to train a $k$-nearest neighbors ($k$-\acro{NN}) binary classifier. This method has the benefit of being non-parametric (hence flexible) and computationally fast to update in light of observations. Building a $k$-\acro{NN} classifier relies on a notion of distance between data points and computing the matrix of $k$ nearest neighbors for every data point given the defined distance formula. This model assumes that every data point $x_i \in \mathcal{D}$ has a binary label $y_i \in \{0, 1\}$. A label of $y_i=1$ means the data point $x_i$ is relevant to the task at hand, whereas a label of $y_i=0$ means $x_i$ is irrelevant. By considering the labels of the nearest neighbors, this model is able to provide us with the probability of any given point being relevant in light of past observations: $\Pr(y_i=1 \mid x_i, \mathcal{I})$. Hence, we use this posterior belief as our relevance function:
\begin{equation}
    f_r(x_i) = \Pr(y_i=1 \mid x_i, \mathcal{I}).
\end{equation}

Monadjemi et al.\cite{monadjemi2020active} used a variation of this modeling technique to maintain a belief over users' latent interest for each attribute. Using a maximum likelihood estimation (\acro{MLE}) approach to computing weights, they merged predictions for each of the attributes to compute the overall relevance value. While their approach performed well in their application, the optimization step for computing the weights becomes prohibitive as the number of attributes grow.

\subsection{Boosted Naive Bayes Classifier}
Healey et al.\cite{healey2012interest} propose a naive Bayes classifier for maintaining a belief over users' interest in data points. In a similar formulation as the $k$-\acro{NN} approach, each data point $x_i \in \mathcal{D}$ has a binary label $y_i \in \{0, 1\}$. A label of $y_i = 1$ means the point $x_i$ is relevant to the task at hand and a label of $y_i = 0$ means it is not relevant. The goal of this approach is to reason about the unknown labels in light of frequencies of observations calculated via the Bayes' law:
\begin{equation}
    \Pr(y_i=1 \mid x_i) \propto \Pr(x_i \mid y_i = 1)\Pr(y_i=1).
\end{equation}
Extending $x_i$ to each of its individual $d$ dimensions and assuming conditional independence among attributes, we get:
\begin{equation}
\begin{split}
        &\Pr(y_i=1 \mid x_{i, 1}, x_{i, 2}, ..., x_{i, d})\\ 
        \propto &\Pr( x_{i, 1}, x_{i, 2}, ..., x_{i, d} \mid y_i = 1)\Pr(y_i=1) \\
        = & \Pr(y_i=1) \prod_{j=1}^{d} \Pr(x_{i,j} \mid y_i=1),
\end{split}
\end{equation}
where $x_{i, j}$ denotes the $j$th attribute of the $i$th data point. Therefore, we get the relevance function as:
\begin{equation}
    f_r(x_i) = \Pr(y_i=1) \prod_{j=1}^{d} \Pr(x_{i,j} \mid y_i=1).
\end{equation}
This model is called \emph{naive} because of the conditional independence assumption among attributes. In more sophisticated models, the dependencies among variable are leaned via techniques called Bayesian structure learning. While Naive Bayes often performs as well as more sophisticated models in practice \cite{langley1992analysis}, its performance can further be improved by \emph{boosting}. As recommended by Healey et al.\cite{healey2012interest}, we also use AdaBoost to train a stronger classifier.


\subsection{Analytic Focus Modeling}
Zhou et al.\cite{zhou2021modeling} propose a technique for modeling analytic focus (\acro{AF}) during a session. Their technique is based on an abstract notion of \emph{concepts} defined as \emph{``meaningful data attribute[s] in the problem domain."} For example, when working with medical literature, concepts can be medical terms appearing in a document. With concepts being left open for practitioners to define in their particular domain, we let each unique value appearing in discrete attributes of the dataset to represent a concept. We perform a pre-processing step on continuous attributes to convert them into discrete bins. The goal of this technique is to track user focus on each of the concepts by observing their interactions and maintain an importance score for each concept. 

As opposed to preceding techniques, \acro{AF} supports different types of interactions. Each interaction $\alpha \in \Alpha$ is defined by two values: an initial importance score $I_\alpha(0)$ and a persistence score $P_\alpha$. In a sense, $I_\alpha(0)$ refers to how intentional an action is and how informative it is in revealing analytic focus. For example, $I_{filter}(0)$ is typically higher than $I_{hover}(0)$ because filtering is often an intentional action taken to focus on a subset of the data whereas hovering can sometimes be unintentional. Moreover, $P_\alpha$ is a measure of how long the visual changes resulting from action $\alpha$ remain. Once again, we expect $P_{filter}$ to be greater than $P_{hover}$ because filtering makes changes to the visualized data until the user reverts the changes, whereas hovering may result in a tooltip opening which will close when the user stops hovering on the point. Using these parameters and the Ebbinghaus forgetting curve [cite], the authors define the per-action importance score function $t$ time steps after an action is taken as: 
\begin{equation}
    I_{\alpha}(t) = I_{\alpha}(0) \times e^{-\frac{t}{P_{\alpha}}}.
\end{equation}
%



Using the equation above, the authors propose an additive model for calculating the importance score for each concept $c$ at time $\tau$:
%
\begin{equation}
    I^c(\tau) = \sum_{(x_{i, t}, \alpha) \in \mathcal{I}_{\tau,c}}I_{\alpha} (\tau - t),
\end{equation}
%
where $\mathcal{I}_{\tau, c}$ denotes the set of interactions with points involving concept $c$ up until time step $\tau$. Considering that each data point $x_i \in \mathcal{D}$ may subscribe to multiple concepts (one concept per dimension in our case), we extent this method so that the importance of a data point is the product of the importance of its individual concepts. In other words, given a data point $x_i \in \mathcal{D}$ and the current time step $\tau$, 
%
\begin{equation}
    f_r(x_i) = \prod_{c \in C(x_i)}{I^c(\tau)},
\end{equation}
%
where $C(x_i)$ is the list of concepts with which $x_i$ is associated.

==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}

\ao{I don't think this section is necessary}
In this section, we narrow the scope of user modeling to learning users' data interest during exploratory analysis. We assume there is a dot-based visualization of a dataset ${\mathcal{D} = \{x_1, x_2, ..., x_n\}}$, where each data point in $\mathcal{D}$ corresponds to a visual element (i.e. a dot) on the visualization. Each data point $x_i \in \mathcal{D}$ has $d$ dimensions (or attributes) which may be continuous, categorical, or ordinal. We denote the set of attributes as ${\mathcal{A} = \{a_1, a_2, ..., a_d\}}$. Due to limitations in visualizing high-dimensional data, only a subset of these attributes may be represented by visual channels on the visualization. 
Users may take different actions while interacting with data points using the visualization. For example, they can filer, zoom, hover, or click. We denote the set of interactions supported by the system as $\Alpha = \{\alpha_1, \alpha_2, ...\}$.
As users interact the visualized data points, we maintain a set of interactions ${\mathcal{I} = \{(x_{i, t}, \alpha)\}}$, where $x_{i, t}$ denotes an interaction of type $\alpha$ with data point $x_i$ at time step $t$.

Consider the following as a running example throughout this section. A user is utilizing Google Maps to determine where to have dinner with a friend. Each restaurant is displayed on the map with visual data attributes such as the star ratings, the type of food, as well as its location (ordinal, categorical, and continuous respectively). We give concrete definitions of two aspects of user modeling related to sessions similar to our motivating example: (i) bias detection and (ii) data ranking.

\subsection{Bias Detection}

The goal of bias detection is to determine if user interactions are biased towards a certain attribute in the dataset. For example, our user may be biased towards location (searching for restaurants in a particular area), food type (looking for Mexican food), ratings (looking for popular and well reviewed places), or any combination of the attributes. Wall et al.\cite{wall2017warning} refer to this type of bias as \emph{attribute distribution} bias. Using a standard notation for every approach considered in this work, we define the \emph{bias function}, $f_{b}$, as follows:
\begin{equation}
    \label{eq:f_bias}
    f_{b} \colon \mathcal{A} \mapsto [0, 1],
\end{equation}
where the set of attributes, $\mathcal{A}$, is mapped to a numerical value between 0 and 1. Higher values correspond to more severe bias towards a certain attribute.

\subsection{Data Ranking}
The goal of data ranking is to learn users' latent interest and rank data points accordingly. Using the example from above, as the user interacts with restaurant points on the map, the data is ranked based on what the algorithm thinks is relevant to the user. We define the \emph{relevance function} as follows:
\begin{equation}
    \label{eq:f_rank}
    f_{r} \colon \mathcal{D} \mapsto [0, 1],
\end{equation}
where the set of data points, $\mathcal{D}$, is mapped to a numerical value between 0 and 1. Higher values correspond data points being more relevant to the task at hand.
Given two data points $x_i, x_j \in \mathcal{D}$, we say $x_i$ is more relevant to the task at hand, $x_i \succ x_j$, if it has a higher relevance value, $f_{r}(x_i) \textgreater f_{r}(x_j)$.

==> tables/datasets.tex <==
\begin{table*}[!ht]
    \centering    \caption{Statistics characterizing the four selected user interaction log datasets.}
    \begin{tabular}{llcccc}
       User Study Data  & Task & \# of Participants & \# of Visual Channels  & \# of Data Attributes & Interaction Type  \\
       \toprule
       STL-location-based \cite{ottley2019follow} & Directed & 28 & 2 & 3 & click\\
       STL-type-based \cite{ottley2019follow} & Directed & 23 & 2 & 3 & click\\
       STL-mixed \cite{ottley2019follow} & Directed & 27 & 2 & 3 & click\\
       \midrule
       Boardrooms \cite{feng2018patterns} & Open-Ended & 39  & 7 & 7 & hover\\
       \midrule
       Vastopolis \cite{monadjemi2020active} & Directed & 123 & 2 & 3 & bookmark\\
       \midrule
       Political Committee \cite{wall2022left} & Directed & 12 & 9 & 9 & bookmark\\
       \bottomrule
    \end{tabular}
    \vspace{5mm}
    \label{tab:user_study_data}
\end{table*}

==> tables/models.tex <==
\begin{table*}[!ht]
    %\footnotesize
    \scriptsize

    \centering
    \caption{Characterizing the seven selected user modeling techniques.}
    \begin{tabular}{llcccc}
       &Modeling Technique  & Bias Detection &  Ranking & Discrete Attributes & Continuous Attributes  \\
       \toprule
       \textbf{HMM}&: Hidden Markov Model \cite{ottley2019follow} & \checkmark &  \checkmark & \checkmark & \checkmark\\
       \midrule
       \textbf{AD}&: Attribute Distribution Bias Metric \cite{wall2017warning} &  \checkmark & $\times$  & \checkmark & \checkmark\\
       \midrule
       \textbf{CM}&: Competing Models \cite{monadjemi2020competing} & \checkmark &  \checkmark & \checkmark & \checkmark\\
       \midrule
       \textbf{AC}&: Adaptive Contextualization \cite{gotz2016adaptive} & \checkmark &  $\times$ & \checkmark & \checkmark\\
       \midrule
       \textbf{$k$-NN}&: $k$-Nearest Neighbors \cite{monadjemi2020active} & $\times$ & \checkmark & \checkmark & \checkmark\\
       \midrule
       \textbf{B-NB}&: Boosted Naive Bayes \cite{healey2012interest} & $\times$ & \checkmark &  \checkmark & $\times$\\
       \midrule
       \textbf{AF}&: Analytic Focus \cite{zhou2021modeling} & $\times$ & \checkmark & \checkmark & $\times$ \\
       \bottomrule
    \end{tabular}
    \vspace{5mm}
    \label{tab:models}
\end{table*}
